Architectural Vulnerability and Reliability Challenges in AI Text Annotation: A Survey-Inspired Framework with Independent Probability Assessment

Large Language Models, despite their power, have a fundamental architectural vulnerability stemming from their causal transformer design -- order sensitivity. This architectural constraint may distorts classification outcomes when prompt elements like label options are reordered, revealing a theoretical gap between accuracy metrics and true model reliability. The paper conceptualizes this vulnerability through the lens of survey methodology, where respondent biases parallel LLM positional dependencies. Empirical evidence using the F1000 biomedical dataset across three scales of LLaMA3.1 models (8B, 70B, 405B) demonstrates that these architectural constraints produce inconsistent annotations under controlled perturbations. The paper advances a practical solution for social science - Independent Probability Assessment - which decouples label evaluation to circumvent positional bias inherent in sequential processing. This approach yields an information-theoretic reliability measure (R-score) that quantifies annotation robustness at the case level. The findings establish that architectural vulnerabilities in causal transformers require methodological innovations beyond accuracy metrics to ensure valid social science inference, as demonstrated through downstream regression analyses where order-sensitive annotations significantly alter substantive conclusions about scientific impact.

==> table1.tex <==
\begin{table}[htbp]
\centering
\caption{Parallels Between Survey Responses and LLM Behavior}
\begin{tabular}{|p{0.3\textwidth}|p{0.3\textwidth}|p{0.3\textwidth}|}
\hline
\textbf{Survey Phenomenon} & \textbf{LLM Parallel} & \textbf{Satisficing Interventions} \\
\hline
Response order effects (primacy, recency) in visual or oral surveys & 
Position/token bias when the model is repeatedly presented with the same label ordering & 
Option randomization to vary the sequence of answer choices \\
\hline
Attention checks and reverse-coded items to ensure consistency & 
Checking consistency across rephrased or negated prompts to detect ``lazy'' or contradictory LLM outputs & 
Reverse validation: Require logical coherence despite altered wording \\
\hline
Framing/context effects: subtle shifts in question wording & 
LLMs can exhibit sensitivity to small changes in prompt context, often yielding superficial or inconsistent answers & 
Position randomization to disrupt any fixed interpretation route \\
\hline
\end{tabular}
\label{table:llm_survey_parallels}
\end{table}

==> table3.tex <==
\begin{table}[htbp]
\centering
\caption{Percentage of Unreliable Cases (KL $\leq$ 0.36) by Model and Category}
\begin{tabular}{lccc}
\hline
\textbf{Model} & \textbf{Interesting Hypothesis} & \textbf{New Finding} & \textbf{Technical Advance} \\
\hline
Llama-3.1-405B & 16.1\% (10/62) & 4.2\% (27/645) & 3.7\% (4/109) \\
Llama-3.1-70B & 12.9\% (8/62) & 10.1\% (65/645) & 5.5\% (6/109) \\
Llama-3.1-8B & 59.7\% (37/62) & 46.2\% (298/645) & 35.8\% (39/109) \\
\hline
\textbf{Overall by Tag} & 29.6\% (55/186) & 20.2\% (390/1935) & 15.0\% (49/327) \\
\hline
\end{tabular}
\label{tab:unreliability}
\end{table}

==> table4.tex <==
\begin{table}[htbp]
\centering
\caption{Overall Unreliability by Model}
\begin{tabular}{lc}
\hline
\textbf{Model} & \textbf{Unreliability Rate} \\
\hline
Llama-3.1-405B & 5.0\% (41/816) \\
Llama-3.1-70B & 9.7\% (79/816) \\
Llama-3.1-8B & 45.8\% (374/816) \\
\hline
\end{tabular}
\label{tab:model_unreliability}
\end{table}
